Modeling Musical Taste Evolution with Recurrent Neural Networks

Finding the music of the moment can often be a challenging problem, even for well-versed music listeners. Musical tastes are constantly in flux, and the problem of developing computational models for musical taste dynamics presents a rich and nebulous problem space. A variety of factors all play some role in determining preferences (e.g., popularity, musicological, social, geographical, generational), and these factors vary across different listeners and contexts. In this paper, we leverage a massive dataset on internet radio station creation from a large music streaming company in order to develop computational models of listener taste evolution. We delve deep into the complexities of this domain, identifying some of the unique challenges that it presents, and develop a model utilizing recurrent neural networks. We apply our model to the problem of next station prediction and show that it not only outperforms several baselines, but excels at long tail music personalization, particularly by learning the long-term dependency structure of listener music preference evolution.

==> OLD-experiments.tex <==
%!TEX root = paper.tex
%
In this section we aim to evaluate the effectiveness of our model for radio station recommendation purpose. After describing our dataset and metrics, we evaluate our model in the task of finding out the next (or the very next one) stations a user will create. 

% \hl{Puya: Assigned to Marta, Puya, Massimo}
% \hl{Puya: Marta please add everything in the wiki page here, }
% \hl{ we need as much volume as possible, ping me when done.}
% %HL
% \noindent\fcolorbox{yellow}{yellow}{
%  \begin{minipage}{0.5\textwidth}
%  Puya:  Regarding the following points:
%  \begin{itemize}
%  \item Trends: is trends a fundamental assumption behind the fact that we use RNN? The answer is NO. you can talk about it, as a way to describe better why RNN is better. But Trends per se, is not a fundamental assumption for us to start using RNN. 
%  \item Evaluation \& Comparison - next-set of stations prediction: nDCG ok (if it doesnt require a lot of time @Marta). 
%  \item Evaluation \& Comparison: Diversity of the results and I would add Robusteness of the recommended stations is something we can add (if there is space); but Marta has already done a lot of experiments.
% Results of our experiments:
%  \item Rephrase: RNN performs better for users that have created in their profile at least 6 stations (active users). 
%  \item RNN is performing better for the task of the very next station prediction. 
%  \item To be fair, we need to apply TDN methodology to all the results (baselines, and our), after the output is generated.
%  \end{itemize}
% \end{minipage}}
% %E-HL
% %\hl{we have to have a section for Time Decay}
% %\hl{we apply it on top of the all the techniques}

\subsection{Dataset}
\label{subsec:dataset}
\begin{figure*}[t!]
\begin{center}
\includegraphics[width=.45\linewidth]{loglog_occurrence}
%\caption{Station creation count distribution.}
%\label{fig:station_cnt_distr}
%\end{figure}
%\begin{figure}
\includegraphics[width=.45\linewidth]{listener_stations}
\caption{On the left distribution of stations creation. On the right distribution of number of stations created by a user.}
\label{fig:dist_stations}
\end{center}
\end{figure*}
 %\mq{Make a new picture. Weird peak at very small x?}

For our experiments, we have collected the data relative to the stations added by a random fraction of the users of a major music streaming platform over a 1-year period. We consider the stations together with the time-stamp in which they have been created. To reduce the impact of the existing recommendation systems used by the platform to suggest new stations to users, we considered only stations added through search-box. While it is still possible that user choices to be influenced by recommendations received in other parts of the application (e.g., while the user listens to her stations), searches through the search-box are clear expressions of the intent of the user of looking for a new station. These are less-biased signals that we believe are good indicator of user interests and hence adequate for modeling the actual interests of the user and their evolution through time.

\begin{table}[th]
\centering
\begin{tabular}{ l | r } 
 \hline \hline
 %Col1 & Col2 \\ 
% \hline
 Number of Listeners & $330,170$ \\ 
 Number of Stations & $3,079,399$ \\
 Number of Listeners (Training) & $324,750$  \\
 Number of Stations (Training) & $2,912,564$  \\
 Number of Listeners (Test) & $64,750$  \\
 Number of Stations (Test) & $151,015$  \\ 
 \hline \hline
\end{tabular}
\caption{Statistics of the Dataset.}
\label{tab:dataset}
\end{table}
\autoref{tab:dataset} reports few details about our dataset. We collected the sequence of stations added by \normaltilde$300$k users over a 1-year period.
\autoref{fig:dist_stations} (on the left) depicts the distribution of station creation. Few stations are used by many people. \autoref{fig:dist_stations} (on the right) depicts distribution of the number of stations created by users. Even that there is a pick, the number of users with few or single stations are compared to the number of users considered is quite low. 

We considered the first 11 months as training and the last month as test dataset\footnote{Notice that this represents only a fraction of the stations actually added by users because of sampling and our restriction to user searches (in other words we do not consider a large amount of stations added by users through recommendation systems)}.
Furthermore, when filter out the stations created by users and not played at least 1 hour (in training). We filter out also users with less than 3 stations.
%in training.%and 20 min in the test set 
%We split the dataset temporally. \mq{Update the rest of this section details on cross-validation} All the events in the first 11 months were used for training the algorithms and the last month for testing. 
Given that a significant fraction of users (\normaltilde 5k) create their first station within the test period, we manually moved their first station into the training set \footnote{This was done to be able to evaluate the recommendation quality also for new users. This does not impact the other methods used in this paper, because none of them uses sequences of length $1$ in training.}. We consider as validation set (to tune our algorithm) a random sample of half of the users in test set.  This fraction of the users was later joined to the training set and the remaining half was used instead exclusively in testing. 


% \begin{table}[t]
% \small
% \centering
% \begin{tabular}{clr}
% \toprule
% \multirow{2}{*}{\textbf{Complete}}&Listeners&330,170\\
% &Stations (unique)&3,079,399 (XXX,XXX)\\
% \midrule
% \multirow{3}{*}{\textbf{Training}}&Listeners&324,750\\
% &Stations (unique)&2,912,564 (98,283)\\
% &Events/station (avg./med.)&29.63/2.0\\
% \midrule
% \multirow{3}{*}{\textbf{Test}}&Listeners (new)&64,750 (5,420)\\
% &Stations (unique)&151,015 (19,827)\\
% &Events/station (avg./med.)&7.62/2.0\\
% \bottomrule
% \end{tabular}
% \caption{Salient characteristics of the dataset \mq{Remove training/test splits and add statistics on the complete dataset}.}
% \label{tab:dataset}
% \end{table}

%\subsection{Evaluation procedures}

\subsection{Metrics}
As evaluation metrics we use standard Information Retrieval
measures. For each user we compute:
\begin{itemize}
\item \emph{MRR}. Reciprocal Rank is the inverse of the position of the first correct station in the ranking produced by the
method.
\item \emph{Recall@K}. The fraction of stations correctly predicted after in $K$ suggestions divided by minimum between $K$ and overall number of stations created by the user in the test set. 
\end{itemize}
To compute the final metrics scores we take the average
of the above measures across all the users.

\subsection{Sequential and Set Evaluation}
As described in Section \ref{subsec:dataset}, our dataset consists of a strictly ordered set of stations created by each user. For the evaluation purpose we consider two cases: \emph{sequential evaluation} and \emph{set evaluation}. In the \emph{sequential evaluation} the stations in test set are considered strictly ordered, while in \emph{set evaluation} we relax this constraint and consider the stations in test set without any particular order.

More formally, let $u$ be a user and $S_u=(s_{u1}, s_{u2}, \ldots, s_{un})$, a list of $n$ stations created by user $u$, $S_u'=(s_{u1}, s_{u2}, \ldots, s_{up})$, $S_u''=(s_{p+1}, s_{p+2}, \ldots, s_{un})$ with $p<n$ respectively be the fraction of $S_u$ considered as training and test, and $R_u$ a ranked list of $K$ station recommendation for user $u$. 
We consider for \emph{set evaluation} the recall for user $u$ to be $\emph{Recall@K}_u= |S_u'' \cap R_u|/min(K,|S_u''|)$ and $\textit{MRR@K}_u$ is inverse rank of the first correct prediction in $R_u$.\\
In \emph{sequential evaluation} the stations in $S_{ui}$ are processed in order. For every station $s_{ui} \in S_u$, a ranked list of $K$ station recommendation $R_{ui}$ is generated; station $s_{ui}$ is then appended to $S_u'$ and removed from $S_u''$. For each list $R_{ui}$, we consider the recall for user $u$ to be $\emph{Recall@K}_{ui}=\mathbb{1}[s_{ui} \in R_{ui}]/K$\footnote{$\mathbb{1}[\cdot]$ is the indicator function.} and $\emph{MRR@K}_{ui}$ to be the inverse rank of $s_{ui}$ if $s_{ui} \in R_{ui}$, 0 otherwise. The metrics are first averaged over every individual user and then averaged over all the users in the dataset.
%\pv{add other cases.}
%We consider instead for \emph{sequential evaluation} the recall to be 
%and $\emph{MRR}_u=$   

%, and  and $S_u''=(s_{u(k+1)}$ respectively be the fraction of $S_u$ considered as training and test. 


%In other words in \emph{sequential evaluation} we want to find the very next station(s) created in the test after right after training, while in \emph{set evaluation} any station created by a user in the test set is considered a positive case.  

\subsection{Baseline and Parameters}
For the baseline we consider (a very naive, unpersonalized) popularity based recommender system (\POP), i.e., recommending always the most popular $K$ stations within the training set.
%This pop recommender always recommends the top$K$ most popular artist or genre on the service. Since our dataset span a full year of user's station creation history, we expect personalized models that better capture users' musical taste evolution to perform better in these metrics.
%\subsection{Model parameters}
We tuned the parameters of each model on the validation set. The optimal configurations for the \RNN\ are hidden layer=$1$, batch size=$500$, batch size=$100$, learning rate=$0.1$, and momentum=$0.1$. While for \KNN\ size=$x$,dumping factor $\lambda$=$x$. In the case of \WTOVEC we consider a context size=$x$, learning rate=$x$, and neighborhood size=$x$.
% \begin{itemize}
% \item \textit{RNN:} hidden layers: 1 (500); batch size: 100; learning rate: 0.1; momentum: 0.1
% \item \textit{Cosine kNN:} neighborhood size: XXX; damping factor $\lambda$: XXX
% \item \textit{Word2Vec kNN:} context size: XXX; learning rate: XXX; neighborhood size: XXX
% \end{itemize}

% \subsection{Evaluation procedures}
% As described in Section \ref{subsec:dataset}, our dataset consists of a strictly ordered set of stations created by each user. For the evaluation purpose we consider two 

% %By splitting the dataset temporally, we end up having a sequence stations in the test set having different length for each user. At this point one important question arises: how should the stations in the test period of every user be considered in the evaluation? This question is closely related with the \textit{order} in which stations are added by users in the test period. Considering the test sequences as unordered or ordered lists leads to very different premises and considerations. For this reason, we devise two different evaluation procedures to analyze this aspect in detail.

% \subsubsection{Set evaluation}
% In \textit{set evaluation} we care about what stations the user will add in future regardless of the order in which she actually adds them to her profile. This is similar to the typical way of evaluating recommender systems, in which we remove a fraction of user's interactions and evaluate the model on how is it capable of predicting all of them. The difference is that stations cannot be held out randomly for the user profile since they where added in a specific temporal order.

% With this type of evaluation, we want to verify whether any information from the sequence of stations added by the user in the past is of any help in predicting the stations that we held out from her profile. This is related with the capability of the recommender of predicting what stations the user will add at any point in future. This can help in building recommendations that are related not only with the immediate interests of the user, but also with the potential developments they can have in future. Still, this type of evaluation is not able to able to dynamically adapt to changes in the user tastes within the test period.

% For each model we generate one ranked list at the beginning of the test period and report metrics. Results are reported in \autoref{tab:set_eval_overall}.
% % \begin{table}[t]
% % \small
% % \centering
% % \begin{tabular}{l|ccc|ccc}
% % \toprule
% % &\multicolumn{3}{c}{\textbf{Recall}}&\multicolumn{3}{c}{\textbf{MRR}}\\
% % $N$&1&5&10&1&5&10\\
% % \midrule
% % RNN&0.0074&0.0273&0.0458&0.0175&0.0308&0.0346\\
% % KNN&0.0074&0.0267&0.0451&0.0183&0.0315&0.0346\\
% % POP&0.0046&0.0153&0.0300&0.0124&0.0211&0.0234\\
% % W2V&0.0041&0.0133&0.0216&0.00975&0.0162&0.0181\\
% % TDSum&\textbf{0.0102}&\textbf{0.0395}&\textbf{0.0673}&\textbf{0.0242}&\textbf{0.0433}&\textbf{0.0479}\\
% % TDMax&x.xxxx&x.xxxx&x.xxxx&x.xxxx&x.xxxx&x.xxxx\\
% % PWF&0.0104&0.0475&0.0593&0.0249&0.0447&0.0455\\
% % \end{tabular}
% % \caption{Overall results for set evaluation}
% % \label{tab:set_eval_overall}
% % \end{table}

% \subsubsection{Sequential evaluation}
% In \textit{sequential evaluation}, we instead care about the order in which users add stations to their profiles. This type of evaluation resembles closely how users actually interact with the system and how recommender systems behave in real-life scenarios. \ty{describe how metrics are calculated here?}

\subsection{Breakdown of Evaluation on Segments}
%\ty{We initially breakdown results by simple user demographic such as age and gender, but they do not reveal insights beyond general trends. Instead we focus on breakdowns on user interaction characteristics and taste evolution.}
To understand better the actual performance of every model we breakdown the evaluation into several evaluation segments.
We initially breakdown results by simple user demographic such as age and gender, but they do not reveal insights beyond general trends. Instead we focus on breakdowns on user interaction characteristics and taste evolution. We consider the following dimensions:
\begin{itemize}
\item{Historical session length}: it corresponds to the number of stations already added by the user at the time of the recommendation. This dimension is used to compare the recommenders in relation to the amount of user's feedback that is available.
\item{User test set size}: it corresponds to the number of stations in the test set. This dimension is used to evaluate the robustness of each recommender to unforeseen drifts in the user interest.
\item{Station popularity}: we subdivided all the stations in the dataset into 4 log-popularity categories \footnote{Station popularity is based on the complete historical listening records of our music streaming service.} We breakdown the evaluation metrics according to the popularity category each station in the test set belongs to. This dimension is used to evaluate how recommenders over different item popularity segments.
\item{User major popularity category}: we categorized users on the popularity category that represents the majority of their listening. This allows to subdivide users that preferably listen to mainstream (short-head) stations from users whose interests span across less popular (long-tail) stations.
\item{User popularity preference}: we further categorized users according to the number of station popularity segments that are needed to collect the 95\% of their listening history. This is a proxy on how a user's interests span different station popularity segments. This is used as further indicator on how the recommender adapts to different degrees of variability in the users' interests. \mq{not 100\% sure about this}
\end{itemize}

%\pv{Add TDK section}

==> OLD-model.tex <==
\para{Time-decayed kNN (TDN).}
To account for the fact that the next-station added by the user may depend not only on the last but also on the sequence of the recently added stations, we propose two different strategies to include the similarity scores of the stations before the last one in the recommendation.

Let $w^{(t)}_j$ be the score of station $j$ at time step $t$. For example, $w^{(t)}_j$ can be the co-occurrence cosine similarity between $j$ and the station added at time $t$. At recommendation time step $T$, the aggregated score $\tilde{w}^{(T)}_j$ is computed by applying one of the following two strategies: (1) Time-decay Sum (TD-Sum), and (2) Time-decay Max (TD-Max). 

Time-decay Sum (TD-Sum) is the weighted sum of the similarity scores received by station $j$ from the starting time step $t_0$ to $T$. Similarity scores are weighed with exponential time decay, and the final score of station $j$ at time step $T$ is computed as
\begin{equation}
\tilde{w}^{(T)}_j = \sum_{t=t_0}^T{\alpha^{T-t} w^{(t)}_j}
\end{equation}
where $\alpha \in [0,1]$ is a temporal decay factor. This corresponds to \textit{reinforcing} $w^{(T)}_j$ with the similarities between station $j$ and stations added by the user in the past, discounted by exponential decay to account for aging effects.

The Time-decay Max (TD-Max) is the maximum weighted similarity scores received by item $j$ from the starting time step $t_0$ to $T$. Similarity scores are weighed with exponential time decay, and the final score of item $j$ at time step $T$ is computed as
\begin{equation}
\tilde{w}^{(T)}_j = \mathrm{max}\left(w^{(T)}_j, \alpha w^{(T-1)}_j, ..., \alpha^{T-t_0} w^{(t_0)}_j\right)
\end{equation}
where $\alpha \in [0,1]$ is a temporal decay factor. This corresponds to assigning to $j$ the maximum similarity score it has with the stations added by the user in the past, discounted with exponential time decay to account for aging effects. This way, a station that is highly similar to a station that is not the immediately last one added by the user has good chances of being recommended.\\

It is worth noting that these strategies can be applied to any similarity-based recommender system. In \cite{grbovic15prod2vec} the authors propose a strategy analogous to TD-Max with exponential decay computed on the actual distance in time (expressed in days) between the the recommendation time and the time of the past user actions. However, in this work we have considered discrete time steps instead of actual time-stamps since user actions are much more sparse in time; users can add new stations few minutes or few months after the last one. %\mq{Is this correct?} In addition, our experiments show that TD-Sum always outperforms TD-Max.

==> OLD-results.tex <==
\begin{figure*}[t!]
\begin{center}
\includegraphics[width=.45\linewidth]{set_general_all_no_tdn_recall}
%\caption{Station creation count distribution.}
%\label{fig:station_cnt_distr}
%\end{figure}
%\begin{figure}
\includegraphics[width=.45\linewidth]{set_general_all_no_tdn_mrr}
\caption{On the left we compare 4 different models in recall. On the right we show the MRR metric.}
\label{fig:set_general_all}
\end{center}
\end{figure*}

\subsection{Model comparison}

First, we perform standard set evaluation on all 4 models for all the users. As shown in \ref{fig:set_general_all},
for the most part, RNN and KNN are similar in recall and MRR metrics, both outperforming prod2vec model and the popularity baseline. We rely on breakdown evaluations to give us further insights into each model's strength and weakness.
\ty{Marta, I think the title on graphs are a bit redundant, perhaps no "+STD error bar"?}


\subsubsection{Breakdown by historical session length}
In \ref{fig:set_seg_hist_no_tdn_recall_1} and \ref{fig:set_seg_hist_no_tdn_recall_5} we can see that RNN underperformed KNN for users with very short historical session length (1 stations), yet outperformed KNN for users with longer history, i.e. more than 6 stations in the last year. When $K>5$, RNN and KNN are similar for users with just a few (2to5) stations. Clearly, for users with limited history, i.e. when a service has little data on a user, a simple KNN can indeed model the next set of music discovery quiet well, beating popularity and prod2vec models. However, when it comes to users with even a relative short history of a few stations, this experiment highlights that Recurrent Neural Network's ability to predict music taste using this history much better than a co-occurrence model KNN. Indeed, in \ref{fig:set_general_gt6_no_tdn_mrr}, we see that RNN outperforms in all $K$ values. This insight is quite encouraging, as it could quantitatively guide recommendation system development to choose suitable recommenders for different users.

In the next sections, we will focus on the set of users that have more than 6 stations in the history, and further study the difference among the models.

\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{set_seg_hist_no_tdn_recall_1}
\caption{Breakdown results by user historical session length, with Recall@1.}
\label{fig:set_seg_hist_no_tdn_recall_1}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{set_seg_hist_no_tdn_recall_5}
\caption{Breakdown results by user historical session length, with Recall@5.}
\label{fig:set_seg_hist_no_tdn_recall_5}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{set_general_gt6_no_tdn_mrr}
\caption{General results for users whose historical session length > 6 stations.}
\label{fig:set_general_gt6_no_tdn_mrr}
\end{center}
\end{figure}

\subsubsection{Breakdown by next session length}
Now we study users by breakdown their behavior in the test set, by the length of their "next session", i.e. number of stations they searched and listened to for a significant amount of time. We observe in \ref{fig:set_seg_next_gt6_no_tdn_mrr_10}, when a recommender is asked to make a large number of recommendation ($K=10$), RNN outperforms KNN and other models in MRR metric. the more stations user create in the next session, the more RNN outperforms. 

\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{set_seg_next_gt6_no_tdn_mrr_10}
\caption{Breakdown by next session length for users whose historical session length > 6 stations.}
\label{fig:set_seg_next_gt6_no_tdn_mrr_10}
\end{center}
\end{figure}


\subsubsection{Breakdown by user popularity preference}
If this is better than station popularity, then we will only show this breakdown

\subsubsection{Difference in results in sequential evaluation}
\ty{2-3 graphs}

\subsection{Model comparison with time decayed scoring}
TDN + description of the method(new plots)

\subsection{Analysis on RNN weights}
Heat maps 


==> results.tex <==
%!TEX root = paper.tex
%

